An Efficient Algorithm For Chinese Postman Walk on Bi-directed de Bruijn Graphs

Sequence assembly from short reads is an important problem in biology. It is known that solving the sequence assembly problem exactly on a bi-directed de Bruijn graph or a string graph is intractable. However finding a Shortest Double stranded DNA string (SDDNA) containing all the k-long words in the reads seems to be a good heuristic to get close to the original genome. This problem is equivalent to finding a cyclic Chinese Postman (CP) walk on the underlying un-weighted bi-directed de Bruijn graph built from the reads. The Chinese Postman walk Problem (CPP) is solved by reducing it to a general bi-directed flow on this graph which runs in O(|E|2 log2(|V |)) time. In this paper we show that the cyclic CPP on bi-directed graphs can be solved without reducing it to bi-directed flow. We present a ?(p(|V | + |E|) log(|V |) + (dmaxp)3) time algorithm to solve the cyclic CPP on a weighted bi-directed de Bruijn graph, where p = max{|{v|din(v) - dout(v) > 0}|, |{v|din(v) - dout(v) < 0}|} and dmax = max{|din(v) - dout(v)}. Our algorithm performs asymptotically better than the bidirected flow algorithm when the number of imbalanced nodes p is much less than the nodes in the bi-directed graph. From our experimental results on various datasets, we have noticed that the value of p/|V | lies between 0.08% and 0.13% with 95% probability.

==> bib1 <==
@article{4russian:1970,
author={Arlazarov,V. L. and Dinic,E. A. and Kronrod,M. A. and Faradzev,I. A.},
year={1970},
title={On economic construction of the transitive closure of a directed graph},
journal={Dokl. Akad. Nauk SSSR},
volume={194},
pages={487-488}
}

@article{tarjan_fibonacci,
author={Fredman,Michael L. and Tarjan,Robert E.},
year={1987},
title={FIBONACCI HEAPS AND THEIR USES IN IMPROVED NETWORK OPTIMIZATION ALGORITHMS.},
journal={Journal of the ACM},
volume={34},
number={3},
pages={596-6l5}
}

@article{hungarian_method,
	author = {Kuhn, H. W. },
			journal = {Naval Research Logistic Quarterly},
					pages = {83--97},
								title = {The {H}ungarian method for the assignment problem},
									volume = {2},
										year = {1955}
}
@article{munkres57,
	author = {Munkres, James  },
			journal = {Journal of the Society for Industrial and Applied Mathematics},
					number = {1},
						pages = {32--38},
									publisher = {SIAM},
										title = {Algorithms for the Assignment and Transportation Problems},
												volume = {5},
													year = {1957}
}
@Article{KuhnH1956Variants,
  author =  {H. W. Kuhn},
    title =  {Variants of the Hungarian method for assignment problems},  
	  journal =  {Naval Research Logistics Quarterly},
	    year =  {1956},
		    volume =  {3},
			    pages =  {253--258}
}






@inproceedings{blum89designing,
 author = "M. Blum and S. Kanna",
 title = {Designing programs that check their work},
 pages = "86--97",
 year = "1989",
}

@article{hirschberg77,
author={Hirschberg,D. S.},
year={1975},
title={Linear Space Algorithm For Computing Maximal Common Subsequences.},
journal={Communications of the ACM},
volume={18},
number={6},
pages={341-343}
}

@inproceedings{nano_raj08,
author={S. Rajasekaran and V. Kumar and S. Sahni and R. Birge},
year={2008},
title={Efficient Algorithms for Protein-Based Associative Processors
and Volumetric Memories},
booktitle={IEEE NANO}
}
@inproceedings{nanomem1,
author={Stuart,Jeffrey A. and Tallent,Jack R. and Tan,Eric H. L. and Birge,Robert R.},
year={1996},
title={Protein-based volumetric memories},
booktitle={Nonvolatile Memory Technology Conference},
pages={45-51}
}

@article{nanomem2,
author={Birge,R. R. and Gillespie,N. B. and Izaguirre,E. W. and Kusnetzow,A. and Lawrence,A. F. and Singh,D. and Song,Q. W. and Schmidt,E. and Stuart,J. A. and Seetharaman,S. and Wise,K. J.},
year={1999},
title={Biomolecular Electronics: Protein-Based Associative Processors and Volumetric Memories},
journal={Journal of Physical Chemistry B},
volume={103},
number={49},
pages={10746-10766}
}









@inproceedings{ukkonen07,
author = "P. Rastas and E. Ukkonen",
title = "Haplotype Inference Via Hierarchical Genotype Parsing",
booktitle = "WABI, LNBI 4645",
pages = "85-97",
year = "2007"
}

@article{aluru03,
author={Rajko,S. and Aluru,S.},
year={2004},
title={Space and time optimal parallel sequence alignments},
journal={IEEE Transactions on Parallel and Distributed Systems},
volume={15},
number={12},
pages={1070-1081}
}

@article{needleman70,
author={Needleman,S. B. and Wunsch,C. D.},
year={1970},
title={A general method applicable to the search for similarities in the amino acid sequence of two proteins.},
journal={Journal of Molecular Biology},
volume={48},
number={3},
pages={443-453}
}

@article{smith81,
				author={Smith,T. F. and Waterman,M. S.},
				year={1981},
				title={Identification of common molecular subsequences.},
				journal={Journal of Molecular Biology},
				volume={147},
				number={1},
				pages={195-197}
}

@article{mayers88,
				author={Myers,E. W. and Miller,W.},
				year={1988},
				title={Optimal alignments in linear space},
				journal={Computer Applications in the Biosciences},
				volume={4},
				number={1},
				pages={11-17}
}

@article{altschul86,
author={Altschul,S. F. and Erickson,B. W.},
year={1986},
title={Optimal sequence alignment using affine gap costs},
journal={Bulletin of Mathematical Biology},
volume={48},
number={5-6},
pages={603-616}
}


@article{gotoh86,
				author={Gotoh,O.},
				year={1986},
				title={Alignment of three biological sequences with an efficient traceback procedure.},
				journal={Journal of Theoretical Biology},
				volume={121},
				number={3},
				pages={327-337}
}

@article{gotoh87,
				author={Gotoh,O.},
				year={1987},
				title={Pattern matching of biological sequences with limited storage},
				journal={Computer Applications in the Biosciences},
				volume={3},
				number={1},
				pages={17-20}
}

@article{huang90,
				author={Huang,X. and Hardison,R. C. and Miller,W.},
				year={1990},
				title={A space-efficient algorithm for local similarities},
				journal={Computer Applications in the Biosciences},
				volume={6},
				number={4},
				pages={373-381}
}


@inproceedings{edmiston87old,
author = "Edmiston E.W. and Wagner R.A.",
title = "Parallelization of the dynamic programming algorithm for comparison of sequences",
booktitle = "Proc. International Conference on Parallel Processing",
pages = "78-80",
year = "1987"
}

@inproceedings{edmiston87,
				        author={Edmiston,Elizabeth and Wagner,Robert A.},
																				        year={1987},
																												        title={PARALLELIZATION OF THE DYNAMIC PROGRAMMING ALGORITHM FOR COMPARISON OF SEQUENCES.},
																																				        pages={78-80}
}

@inproceedings{edmiston88,
				        author={Core,Nolan G. and Edmiston,Elizabeth W. and Saltz,Joel H. and Smith,Roger M.},
												        year={1988},
																				        title={Parallel processing of biological sequence comparison algorithms},
																												        pages={266-270}
}

@article{ranka90,
 author={Ranka,Sanjay and Sahni,Sartaj},
     year={1990},
       title={String editing on an SIMD hypercube multicomputer},
     journal={Journal of Parallel and Distributed Computing},
       volume={9},
        number={4},
        pages={411-418}
}


@book{gusfield97,
author = "Gusfield,Dan",
title = "Algorithms of Strings Trees and Sequences",
publisher = "Cambridge",
pages = "302-308",
year ="1997"
}
@inproceedings{knuth2,
author = "Donald,Knuth",
title = "Art of Computer Programming: Volume 2",
publisher = "Pearson Education",
pages = "204-205",
year = "1999"
}

@book{hsr08,
author = "Horowitz,Ellis and Sahni,Satraj and Rajasekaran,Sanguthevar",
title = "Computer Algorithms",
publisher = "Silicon Press",
year = "2008"
}

@inproceedings{raj08,
author = "Rajasekaran S. and Sen S.",
title = "Optimal and Practical Algorithms for Sorting on the PDM",
booktitle = "IEEE Transactions on Computers",
year = "April,2008"
}

@inproceedings{mckay78,
author = "Brendan D. McKay",
title = "Computing AUtomorphishms and Canonical Labelling of Graphs",
booktitle = "Combinatorial Mathematics",
pages = "223-232",
year = "Volume 686/1978"
}

@inproceedings{ullmann76,
author = "Ullmann J.R.",
title = "An Algorithm for Subgraph Isomorphism",
booktitle = "Journal of the ACM (JACM)",
pages = "31-42",  
year = " Volume 23 ,  Issue 1  (January 1976)"
}

@inproceedings{corneil70,
author = "Corneil D.G. and Gotlieb C.C.",
title = "An Efficient Algorithm for Graph Isomorphism",
booktitle = "Journal of the ACM (JACM)",
pages = "51-64",  
year = " Volume 17 ,  Issue 1  (January 1970)"
}

@inproceedings{babai82,
author = "Babai L. and Grigoryev and Yu D. and Mount D.",
title = "Isomorphism of graphs with bounded eigen value multiplicity",
booktitle = "Proceedings of the 14th Annual ACM Symposium on Theory of Computing",
pages = "310-324",
year = "1982"
}

@inproceedings{Har62,
author = "Harary F.",
title = "THe determinant of the adjacency matrix of a graph",
booktitle = "SIAM Review",
pages = "202-210",
year = "Vol.4, 1962"
}

@inproceedings{CRS97,
author = "Cvetkovi\'{c} D. and Rowlingson P. and Simi\'{c} S.",
title = "Eigenspaces of Graphs",
booktitle = "Cambridge University Press",
year = "1997"
}

@inproceedings{GoMc82,
author = "Godsil C.D. and McKay B.D.",
title = "Constructing cospectral graphs",
booktitle ="Acquationes Mathematicae",
pages = "257-268",
year = "2001"
}

@inproceedings{Sch73,
author = "Schwenk A.J.",
title = "Almost all trees are cospectral",
booktitle = "New Directions in the Theory of Graphs (Proc. Third Annual Arbor Conference)",
pages = "275-307",
year = "1973"
}

@inproceedings{Mck81,
author = "McKay B.D.",
title = "Practical Graph Isomorphism",
booktitle = "Congressus Numerantium",
pages = "45-87",
year = "1981"
}

@inproceedings{unger64,
author = "Unger S.H.",
title = "GIT -- A heuristic program for testing pairs of directed line graphs 
for isomorphism",
booktitle = "Comm. ACM",
pages = "26-43",
year = "Jan, 1964"
}




@inproceedings{SPLASH, 
author = "D. T. Hoang",
title = "Searching Genetic Databases on {SPLASH} 2",
booktitle = "{IEEE} WkShp on {FPGA}s for Custom Computing Machines",
pages = "185--191",
year = "1993"
}

@techreport{hoang92,
author = "D. T. Hoang",
title = "A Systolic Array for the Sequence Alignment Problem",
number = "CS-92-22",
year = "1992"
}

@article{CASM,
author = "R. Sastry and N. Ranganathan and K. Remedios",
title = "{CASM}: {A VLSI} Chip for Approximate String Matching",
journal = {IEEE Trans. Pattern Anal. Mach. Intell.},
volume = {17},
number = {8},
year = {1995},
pages = {824--830},
publisher = {IEEE Computer Society},
address = {Washington, DC, USA},
}

@inproceedings{sastry93,
author = {R. Sastry and N. Ranganathan},
title = {A systolic array for approximate string matching},
booktitle = {Int. Conf. Computer Design},
pages = "402-405",
year = "1993"
}

@article{cheng87,
author = {H. D. Cheng and K. S. Fu},
title = "{VLSI} architectures for string matching and pattern matching",
journal = {Pattern Recogn.},
volume = {20},
number = {1},
year = {1987},
pages = {125--144},
publisher = {Elsevier Science Inc.},
address = {New York, NY, USA},
}

@article{PNAC,
author = {D. P. Lopresti},
title = "{P-NAC: A} Systolic Array for Comparing Nucleic Acid Sequences",
journal = {Computer},
volume = {20},
number = {7},
year = {1987},
pages = {98--99},
publisher = {IEEE Computer Society Press},
address = {Los Alamitos, CA, USA},
}

@article{fpga1,
author = "P. D. Michailidis and K. G. Margaritis",
title = {A programmable array processor architecture for flexible approximate string matching algorithms},
journal = {J. Parallel Distrib. Comput.},
volume = {67},
number = {2},
year = {2007},
pages = {131--141},
publisher = {Academic Press, Inc.},
address = {Orlando, FL, USA},
}

@article{fpga2,
author = "M. C. Herbordt and J. Model and B. Sukhwani and Y. Gu and T. VanCourt",
title = "{Single pass streaming BLAST on FPGAs}",
journal = {Parallel Comput.},
volume = {33},
number = {10-11},
year = {2007},
pages = {741--756},
publisher = {Elsevier Science Publishers B. V.},
address = {Amsterdam, The Netherlands, The Netherlands},
}



@article{mukherjee89,
author = {A. Mukherjee},
title = {Hardware Algorithms for Determining Similarity Between two Strings},
journal = {IEEE Trans. Comput.},
volume = {38},
number = {4},
year = {1989},
pages = {600--603},
publisher = {IEEE Computer Society},
address = {Washington, DC, USA},
}


@inproceedings{lipton85,
author = "R. J. Lipton and D. Lopresti",
title = "A systolic array for rapid string comparison",
booktitle = "Chapel Hill Conf. on VLSI",
pages ="363-376",
year ="1985"
}

@article{blast,
author = "S. F. Altschul and W. Gish and W. Miller and E. W. Myers and D. J. Lipman",
title = "Basic Local Alignment Search Tool",
journal="J. Mol. Biol.",
volume="215",
pages = "403-410",
year = "1990"
}


@book{algos_text,
author = "T.  H.  Cormen and C.  E. Leiserson and R. L. Rivest and C. Stein",
title = {Introduction to Algorithms, Second Edition},
publisher = {The MIT Press},
month = {Sept.},
year = {2001}
}


@book{durbin99,
author="R. Durbin and S. R. Eddy and A. Krog and G. Mitchison",
title = "Biological Sequence Analysis: Probabilistic Models of
Proteins and Nucleic Acids",
publisher = "Cambridge University Press",
year = "1999"
}

@misc{ansoft_nexxim,
title="NEXXIM Ansoft circuit simulator",
note="[\texttt{http://www.ansoft.com/}]"
}

@misc{homepage,
title="{Circuit Design for EditDistance}",
note="[Suppressed for paper blind review.]"
}
@misc{home_page,
title={Home Page},
note="[\texttt{http://dna.engr.uconn.edu/~vamsik}]"
}

@misc{synopsys,
title="{Synopsys Design and Simulation Tools}",
note="[\texttt{http://www.synopsys.com}]"
}
@misc{intel_ext,
title = "{Intel instruction set extensions(SMID) for Multimedia streaming}",
note="[\texttt{ftp://download.intel.com/technology/itj/Q21999/PDF/simd_ext.pdf}]"
}

@misc{fuse,
title="{File System in Userspace}",
note="[\texttt{http://fuse.sf.net}]"
}
@misc{postmark,
title="{PostMark Benchmark}",
note="[\texttt{http://www.devone.org/linux/postmark.html}]"
}
@misc{iozone,
title="{IOZone File System Benchmark}",
note="[\texttt{http://www.iozone.org}]"
}

@inproceedings{abraham05,
AUTHOR = {Abraham, David J. and Irving, Robert W. and Kavitha,
		  Telikepalli and Mehlhorn, Kurt},
TITLE = {Popular matchings},
BOOKTITLE = {Proceedings of the {S}ixteenth {A}nnual {ACM}-{SIAM}
							  {S}ymposium on {D}iscrete {A}lgorithms},
PAGES = {424--432 (electronic)},
PUBLISHER = {ACM},
ADDRESS = {New York},
YEAR = {2005},
MRCLASS = {91B68 (05D15)},
MRNUMBER = {MR2298291},
}
@incollection{mestre06,
AUTHOR = {Mestre, Juli{\'a}n},
TITLE = {Weighted popular matchings},
BOOKTITLE = {Automata, languages and programming. {P}art {I}},
SERIES = {Lecture Notes in Comput. Sci.},
VOLUME = {4051},
PAGES = {715--726},
PUBLISHER = {Springer},
ADDRESS = {Berlin},
YEAR = {2006},
MRCLASS = {05C70 (90C27)},
MRNUMBER = {MR2305570},
}
@article{gardenfors75,
	author={GARDENFORS,P.},
	year={1975},
	title={MATCH MAKING: ASSIGNMENTS BASED ON BILATERAL PREFERENCES},
	journal={Behavioral Science},
	volume={20},
	number={3},
	pages={166-173}
}

@inproceedings{kavitha08,
author={Telikepalli Kavitha and Meghana Nasre},
year={2008},
title={Optimal Popular Matching},
booktitle={MATCH-UP (http://www.optimalmatching.com/workshop)}
}
%
%
% Adding references for the BLMP paper.
%
@INPROCEEDINGS{CAR-RAH-2006,
AUTHOR = {de Carvalho Jr., S.A. and S. Rahmann},
TITLE = {Improving the layout of oligonucleotide microarrays: {Pivot Partitioning}},
BOOKTITLE = {Proc. 6th Workshop of Algorithms in Bioinformatics},
YEAR = {2006},
VOLUME = {4175},
SERIES = {LNBI},
PAGES = {321--332},
NOEDITOR = {Philipp Bucher and Bernard Moret},
OPTPUBLISHER = {Springer},
OWNER = {heike},
TIMESTAMP = {2007.01.15}
}

@inproceedings{cindy2008,
author={Cindy Y. Li and Prudence W. H. Wong and Qin Xin and Fencol C. C. Yung},
title={Approximating Border Length for DNA Microarray Synthesis},
booktitle={Theory and Applications of Models of Computation},
year={2008},
pages={410-422}

}

@inproceedings{kundetibibe2009,
author= {V. Kundeti and S. Rajasekaran},
TITLE={On the hardness of the border length minimization problem},
booktitle = {IEEE International conference on bioinformatics and bio-engineering},
year={2009},
pages={248-253}
}

@inproceedings{CAR-RAH-2006a,
AUTHOR = {de Carvalho Jr., S.A. and S. Rahmann},
TITLE = {Microarray layout as a quadratic assignment problem},
BOOKTITLE = {Proc. German Conference on Bioinformatics},
YEAR = {2006},
VOLUME = {P-83},
SERIES = {Lecture Notes in Informatics},
PAGES = {11--20},
NOEDITOR = {Daniel Huson and Oliver Kohlbacher and Andrei Lupas and 
Kay Nieselt and Andreas Zell},
OPTPUBLISHER = {GI},
OWNER = {heike},
TIMESTAMP = {2007.01.15}
}

@article{hannenhalli96,
author={Hannenhalli,S. and Hubell,E. and Lipshutz,R. and Pevzner,P. A.},
year={2002},
title={Combinatorial algorithms for design of DNA arrays.},
journal={Advances in biochemical engineering/biotechnology},
volume={77},
pages={1-19}
}

@inproceedings{epitaxial03,
author = {Kahng, Andrew B. and Mandoiu, Ion I. and Pevzner, Pavel A. and Reda, Sherief and Zelikovsky, Alexander},
title = {Border Length Minimization in DNA Array Design},
booktitle = {WABI '02: Proceedings of the Second International Workshop on Algorithms in Bioinformatics},
year = {2002},
isbn = {3-540-44211-1},
pages = {435--448},
publisher = {Springer-Verlag},
address = {London, UK},
}


@article{BGI+99,
author={Birge,R. R. and Gillespie,N. B. and Izaguirre,E. W. and Kusnetzow,A. and Lawrence,A. F. and Singh,D. and Song,Q. W. and Schmidt,E. and Stuart,J. A. and Seetharaman,S. and Wise,K. J.},
year={1999},
title={Biomolecular Electronics: Protein-Based Associative Processors and Volumetric Memories},
journal={Journal of Physical Chemistry B},
volume={103},
number={49},
pages={10746-10766}
}

@article{Ham00,
author={Hampp,N. A.},
year={2000},
title={Bacteriorhodopsin: Mutating a biomaterial into an optoelectronic material},
journal={Applied Microbiology and Biotechnology},
volume={53},
number={6},
pages={633-639}
}

@article{HKW+05,
author={Hillebrecht,J. R. and Koscielecki,J. F. and Wise,K. J. and Marcy,D. L. and Tetley,W. and Rangarajan,R. and Sullivan,J. and Brideau,M. and Krebs,M. P. and Stuart,J. A. and Birge,R. R.},
year={2005},
title={Optimization of protein-based volumetric optical memories and associative processors by using directed evolution},
journal={Nanobiotechnology},
volume={1},
number={2},
pages={141-151}
}

@article{WGS+02,
author={Wise,K. J. and Gillespie,N. B. and Stuart,J. A. and Krebs,M. P. and Birge,R. R.},
year={2002},
title={Optimization of bacteriorhodopsin for bioelectronic devices},
journal={Trends in Biotechnology},
volume={20},
number={9},
pages={387-394}
}

@article{ashleyIBM00,
author={Ashley,J. and Bernal,M. -. and Burr,G. W. and Coufal,H. and Guenther,H. and Hoffnagle,J. A. and Jefferson,C. M. and Marcus,B. and Macfarlane,R. M. and Shelby,R. M. and Sincerbox,G. T.},
year={2000},
title={Holographic data storage},
journal={IBM Journal of Research and Development},
volume={44},
number={3},
pages={341-368},
}









@article{Bir90,
author={Birge,R. R.},
year={1990},
title={Photophysics and molecular electronic applications of the rhodopsins},
journal={Annual Review of Physical Chemistry},
volume={41},
number={1},
pages={683-733}
}
@article{hammingtsp,
author={Ernvall,J. and Katajainen,J. and Penttonen,M.},
year={1985},
title={NP-completeness of the hamming salesman problem},
journal={BIT},
volume={25},
number={1},
pages={289-292}
}
@article{optmem05,
author={Hillebrecht,J. R. and Koscielecki,J. F. and Wise,K. J. and Marcy,D. L. and Tetley,W. and Rangarajan,R. and Sullivan,J. and Brideau,M. and Krebs,M. P. and Stuart,J. A. and Birge,R. R.},
year={2005},
title={Optimization of protein-based volumetric optical memories and associative processors by using directed evolution},
journal={Nanobiotechnology},
volume={1},
number={2},
pages={141-151}
}


@article{6:8_code,
author={Burr,G. W. and Ashley,J. and Coufal,H. and Grygier,R. K. and Hoffnagle,J. A. and Jefferson,C. M. and Marcus,B.},
year={1997},
title={Modulation coding for pixel-matched holographic data storage},
journal={Optics Letters},
volume={22},
number={9},
pages={639-641}
}

@article{LZW,
author={Ziv,Jacob and Lempel,Abraham},
year={1978},
title={COMPRESSION OF INDIVIDUAL SEQUENCES VIA VARIABLE-RATE CODING.},
journal={IEEE Transactions on Information Theory},
volume={IT-24},
number={5},
pages={530-536}
}

@inproceedings{MStateRealTime,
author={Hampp,N. and Juchem,T.},
year={2001},
title={System for holographic interferometry based on bacteriorhodopsin films},
booktitle={Proceedings of SPIE - 4597},
volume={4597},
pages={7-15}
}


@article{QStateLongLived,
author={Birge,R. R. and Gillespie,N. B. and Izaguirre,E. W. and Kusnetzow,A. and Lawrence,A. F. and Singh,D. and Song,Q. W. and Schmidt,E. and Stuart,J. A. and Seetharaman,S. and Wise,K. J.},
year={1999},
title={Biomolecular Electronics: Protein-Based Associative Processors and Volumetric Memories}, 
journal={Journal of Physical Chemistry B},
volume={103},
number={49},
pages={10746-10766},
}

@article{google98,
author={Brin,S.},
year={1998},
title={The anatomy of a large-scale hypertextual Web search engine 1},
journal={Computer Networks},
volume={30},
number={1-7},
pages={107-117}
}


@article{HITS99,
author={Kleinberg,J. M.},
year={1999},
title={Authoritative sources in a hyperlinked environment},
journal={Journal of the ACM},
volume={46},
number={5},
pages={604-632}
}

@inproceedings{relayplacement06,
author={Kashyap,A. and Khuller,S. and Shayman,M.},
year={2006},
title={Relay placement for higher order connectivity in wireless sensor networks},
booktitle={in Proceedings of IEEE Infocom}
}
@INPROCEEDINGS{datacollection03,
author = {William C. Cheng and Cheng-fu Chou and Leana Golubchik and Samir Khuller},
title = {Largescale data collection: a coordinated approach},
booktitle = {in Proceedings of IEEE INFOCOM},
year = {2003},
pages = {218--228}
}

%
% References for the preordering paper
%

@article{Hagemann06,
	author={Hagemann,M. and Schenk,O.},
	year={2006},
	title={Weighted matchings for preconditioning symmetric indefinite linear systems},
	journal={SIAM Journal of Scientific Computing},
	volume={28},
	number={2},
	pages={403-420}
}

@article{Duff01,
	author={Duff,I. S. and Koster,J.},
	year={2001},
	title={On algorithms for permuting large entries to the diagonal of a sparse matrix},
	journal={SIAM Journal on Matrix Analysis and Applications},
	volume={22},
	number={4},
	pages={973-996}
}

@ARTICLE{Li03superludist,
author = {Xiaoye S. Li and James W. Demmel},
title = {SuperLU DIST: A scalable distributed-memory sparse direct solver for unsymmetric linear systems},
journal = {ACM Transactions on Mathematical Software},
year = {2003},
volume = {29},
pages = {110--140}
}

@article{PROSITE,
author={Bairoch,A.},
year={1991},
title={PROSITE: a dictionary of sites and patterns in proteins},
journal={Nucleic Acids Research},
volume={19},
number={SUPPL.},
pages={2241-2245}
}

@article{MnM1,
author={Balla,S. and Thapar,V. and Verma,S. and Luong,T. and Faghri,T. and Huang,C. H. and Rajasekaran,S. and del Campo,J. J. and Shinn,J. H. and Mohler,W. A. and Maciejewski,M. W. and Gryk,M. R. and Piccirillo,B. and Schiller,S. R. and Schiller,M. R.},
year={2006},
title={Minimotif Miner: a tool for investigating protein function.},
journal={Nature methods.},
volume={3},
number={3},
pages={175-177}
}

@article{yatesNFA,
author={Baeza-Yates,R. and Navarro,G.},
year={1999},
title={Faster approximate string matching},
journal={Algorithmica (New York)},
volume={23},
number={2},
pages={127-158}
}

@book{HyyroNFA,
author={Hyyrö,H.},
year={2006},
title={Tighter packed bit-parallel NFA for approximate string matching},
volume={4094 LNCS},
pages={287-289}
}

@article{MnM2,
abstract = {Minimotif Miner (MnM) consists of a minimotif database and a web-based application that enables prediction of motif-based functions in user-supplied protein queries. We have revised MnM by expanding the database more than 10-fold to approximately 5000 motifs and standardized the motif function definitions. The web-application user interface has been redeveloped with new features including improved navigation, screencast-driven help, support for alias names and expanded SNP analysis. A sample analysis of prion shows how MnM 2 can be used. Weblink: http://mnm.engr.uconn.edu, weblink for version 1 is http://sms.engr.uconn.edu.},
author = {Rajasekaran, Sanguthevar   and Balla, Sudha   and Gradie, Patrick   and Gryk, Michael R  R.  and Kadaveru, Krishna   and Kundeti, Vamsi   and Maciejewski, Mark W  W.  and Mi, Tian   and Rubino, Nicholas   and Vyas, Jay   and Schiller, Martin R  R. },
issn = {1362-4962},
journal = {Nucleic acids research},
month = {October},
title = {Minimotif miner 2nd release: a database and web system for motif search.},
url = {http://view.ncbi.nlm.nih.gov/pubmed/18978024},
year = {2008}
}


@article{aho-corasick,
author={Aho,Alfred V. and Corasick,Margaret J.},
year={1975},
title={EFFICIENT STRING MATCHING: AN AID TO BIBLIOGRAPHIC SEARCH.},
journal={Communications of the ACM},
volume={18},
number={6},
pages={333-340}
}

@article{thompsonNFA,
author={Thompson,K.},
year={1968},
title={Regular expression search algorithm},
journal={Communications of the ACM},
volume={11},
number={6},
pages={419-422}
}

@article{winfree,
author={Soloveichik,D. and Winfree,E.},
year={2007},
title={Complexity of self-assembled shapes},
journal={SIAM Journal on Computing},
volume={36},
number={6},
pages={1544-1569}
}

@inproceedings{RothemundSTOC,
author={Rothemund,P. W. K. and Winfree,E.},
year={2000},
title={Program-size complexity of self-assembled squares},
booktitle={ACM Symposium on Theory Of Computation (STOC)},
pages={459-468}
}

@article{SeemanDNA,
author={Seeman,N. C.},
year={1982},
title={Nucleic acid junctions and lattices},
journal={Journal of Theoretical Biology},
volume={99},
number={2},
pages={237-247}
}

@article{Seeman03,
author={Seeman,N. C.},
year={2003},
title={Biochemistry and structural DNA nanotechnology: An evolving symbiotic relationship},
journal={Biochemistry},
volume={42},
number={24},
pages={7259-7269},
}

@article{WangsTiling,
author={Wang,H.},
year={1962},
title={An unsolvable problem on dominoes},
journal={Technical Report},
volume={BL-30}
}

@article{reif_dna_computation,
author={Reif,J. H.},
year={1999},
title={Local parallel biomolecular computation},
journal={DNA Based Computers III},
volume={48},
pages={217-254}
}


@article{adleman_seminal,
author={Adleman,L. M.},
year={1994},
title={Molecular computation of solutions to combinatorial problems},
journal={Science},
volume={266},
number={5187},
pages={1021-1024}
}

@article{triple_crossover_tiles,
author={Mao,C. and LaBean,T. H. and Reif,J. H. and Seeman,N. C.},
year={2000},
title={Logical computation using algorithmic self-assembly of DNA triple-crossover molecules},
journal={Nature},
volume={407},
number={6803},
pages={493-496},
}

@article{labean_triple,
author={LaBean,T. H. and Yan,H. and Kopatsch,J. and Liu,F. and Winfree,E. and Reif,J. H. and Seeman,N. C.},
year={2000},
title={Construction, analysis, ligation, and self-assembly of DNA triple crossover complexes},
journal={Journal of the American Chemical Society},
volume={122},
number={9},
pages={1848-1860}
}

@article{DNACrystals,
author={Winfree,E. and Liu,F. and Wenzler,L. A. and Seeman,N. C.},
year={1998},
title={Design and self-assembly of two-dimensional DNA crystals},
journal={Nature},
volume={394},
number={6693},
pages={539-544}
}

@article{gates_self_assembly,
author={Huang,Y. and Duan,X. and Cui,Y. and Lauhon,L. J. and Kim,K. -. and Lieber,C. M.},
year={2001},
title={Logic gates and computation from assembled nanowire building blocks},
journal={Science},
volume={294},
number={5545},
pages={1313-1317}
}

@article{cook_circuit,
author={Cook,M. and Rothemund,P. W. K. and Winfree,E.},
year={2004},
title={Self-assembled circuit patterns},
journal={LNCS},
volume={2943},
pages={91-107}
}

@article{scalable_self_assembly,
author={LaBean,T. H. and Winfree,E. and Reif,J. H.},
year={2000},
title={Experimental progress in computation by self-assembly of DNA tilings},
journal={Proc. DNA Based Computers},
volume={54},
pages={123-140}
}

@article{nano_gates,
author={Bachtold,A. and Hadley,P. and Nakanishi,T. and Dekker,C.},
year={2001},
title={Logic circuits with carbon nanotube transistors},
journal={Science},
volume={294},
number={5545},
pages={1317-1320}
}

@article{assembly_model1,
author={Aggarwal,G. and Cheng,Q. I. and Goldwasser,M. H. and Kao,M. -. and De Espanes,P. M. and Schweller,R. T.},
year={2005},
title={Complexities for generalized models of self-assembly},
journal={SIAM Journal on Computing},
volume={34},
number={6},
pages={1493-1515}
}

@book{random_model1,
author={Kao,M. -. and Schweller,R.},
year={2008},
title={Randomized self-assembly for approximate shapes},
volume={5125 LNCS},
number={PART 1},
pages={370-384},
}

@inproceedings{assembly_model2,
author={Kao,M. -. and Schweller,R.},
year={2006},
title={Reducing tile complexity for self-assembly through temperature programming},
pages={571-580},
booktitle={Annual ACM-SIAM Symposium on Discrete Algorithms}
}





@inproceedings{adlemanSTOC,
author={Adleman,L. and Cheng,Q. and Goel,A. and Huang,M. -.},
year={2001},
title={Running time and program size for self-assembled squares},
pages={740-748},
booktitle={Annual ACM Symposium on Theory of Computing}
}


@inproceedings{SA-ASAP,
author={Kundeti,V. and Fei,Y. and Rajasekaran,S.},
year={2008},
title={An efficient digital circuit for implementing sequence alignment algorithm in an extended processor},
booktitle={IEEE ASAP},
pages={156-161}
}

@inproceedings{SAPE,
author={Kundeti,V. and Rajasekaran,S.},
year={2008},
title={Local Structural Alignment With Variable Length Alignment Fragment Pairs},
booktitle={IEEE BIBE}
}

@book{ED-ICCS,
author={Kundeti,V. and Rajasekaran,S.},
year={2008},
title={Extending the four Russian algorithm to compute the edit script in linear space},
volume={5101 LNCS},
number={PART 1},
pages={893-902}
}

@article{JMMA-VLSI,
author={Kundeti,V. K. and Gupta,P.},
year={2006},
title={Optimal algorithms for some polygon enclosure problems for VLSI Layout Analysis},
journal={Journal of Mathematical Modelling and Algorithms},
volume={5},
number={3},
pages={259-271}
}

@inproceedings{PDM-HiPC,
title = {Efficient PDM Sorting Algorithms.},
author = {Vamsi Kundeti and Sanguthevar Rajasekaran},
booktitle = {HiPC},
editor = {P. Sadayappan and Manish Parashar and Ramamurthy Badrinath and Viktor K. Prasanna},
pages = {97-107},
publisher = {Springer},
series = {Lecture Notes in Computer Science},
volume = {5374},
year = {2008}
}

@article{welsh2003,
	author={Welsh,J. B. and Sapinoso,L. M. and Kern,S. G. and Brown,D. A. and Liu,T. and Bauskin,A. R. and Ward,R. L. and Hawkins,N. J. and Quinn,D. I. and Russell,P. J. and Sutherland,R. L. and Breit,S. N. and Moskaluk,C. A. and Frierson Jr.,H. F. and Hampton,G. M.},
	year={2003},
	title={Large-scale delineation of secreted protein biomarkers overexpressed in cancer tissue and serum},
	journal={Proceedings of the National Academy of Sciences of the United States of America},
	volume={100},
	number={6},
	pages={3410-3415}
}

@article{pistkun2006,
	author={Pisitkun,T. and Johnstone,R. and Knepper,M. A.},
	year={2006},
	title={Discovery of urinary biomarkers},
	journal={Molecular and Cellular Proteomics},
	volume={5},
	number={10},
	pages={1760-1771}
}
}

@article{chatterjee2006,
	author={Chatterjee,M. and Mohapatra,S. and Ionan,A. and Bawa,G. and Ali-Fehmi,R. and Wang,X. and Nowak,J. and Ye,B. and Nahhas,F. A. and Lu,K. and Witkin,S. S. and Fishman,D. and Munkarah,A. and Morris,R. and Levin,N. K. and Shirley,N. N. and Tromp,G. and Abrams,J. and Draghici,S. and Tainsky,M. A.},
	year={2006},
	title={Diagnostic markers of ovarian cancer by high-throughput antigen cloning and detection on arrays},
	journal={Cancer research},
	volume={66},
	number={2},
	pages={1181-1190}
}
}

@article{melle2004,
	author={Melle,C. and Ernst,G. and Schimmel,B. and Bleul,A. and Koscielny,S. and Wiesner,A. and Bogumil,R. and Möller,U. and Osterloh,D. and Halbhuber,K. -. and Von Eggeling,F.},
	year={2004},
	title={A technical triade for proteomic identification and characterization of cancer biomarkers},
	journal={Cancer research},
	volume={64},
	number={12},
	pages={4099-4104}
}

@article{kolch2005,
	author={Kolch,W. and Mischak,H. and Pitt,A. R.},
	year={2005},
	title={The molecular make-up of a tumour: Proteomics in cancer research},
	journal={Clinical science},
	volume={108},
	number={5},
	pages={369-383}
}

@article{1.5-approx-HTSP,
author={Nicos Christofides},
year={1976},
title={Worst-case analysis of a new heuristic for the travelling salesman problem},
journal={Graduate School of Industrial Administration},
volume={Report 388}
}

@article{velvet08,
author={Zerbino,D. R. and Birney,E.},
year={2008},
title={Velvet: Algorithms for de novo short read assembly using de Bruijn graphs},
journal={Genome research},
volume={18},
number={5},
pages={821-829}
}


@book{bidirected_graph,
author={Medvedev,P. and Georgiou,K. and Myers,G. and Brudno,M.},
year={2007},
title={Computability of models for sequence assembly},
volume={4645 LNBI},
pages={289-301}
}

@inproceedings{par_bidirected_graph,
author={Jackson,B. G. and Aluru,S.},
year={2008},
title={Parallel construction of bidirected string graphs for genome assembly},
pages={346-353}
}
@article{myers95,
author={Kececioglu,J. D. and Myers,E. W.},
year={1995},
title={Combinatorial algorithms for DNA sequence assembly},
journal={Algorithmica},
volume={13},
number={1-2},
pages={7-51}
}


@article{myers05,
author={Myers,E. W.},
year={2005},
title={The fragment assembly string graph},
journal={Bioinformatics},
volume={21},
number={SUPPL. 2},
pages={ii79-ii85}
}

@article{pevzner01,
author={Pevzner,P. A. and Tang,H. and Waterman,M. S.},
year={2001},
title={An Eulerian path approach to DNA fragment assembly},
journal={Proceedings of the National Academy of Sciences of the United States of America},
volume={98},
number={17},
pages={9748-9753}
}

@misc{cplex,
title="{ILOG Software}",
note="[\texttt{http://www.ilog.com/products/cplex}]"
}

%
%
% Adding references for the BLMP paper.
%

@article{dnasynthesis,
author={Fodor,S. P. A. and Read,J. L. and Pirrung,M. C. and Stryer,L. and Lu,A. T. and Solas,D.},
year={1991},
title={Light-directed, spatially addressable parallel chemical synthesis},
journal={Science},
volume={251},
number={4995},
pages={767-773}
}

@inproceedings{cec_codes,
author={Kundeti,V. and Rajasekaran,S. and Birge,R.},
year={2009},
title={Generalized algorithms for generating balanced modulation codes in protein-based volumetric memories},
booktitle={10th IEEE International Conference on Evolutionary Computation (CEC)},
pages={1585-1590},
}
@unpublished{bi-graph-out-core,
author={Kundeti,V. and Rajasekaran,S. and Dinh,H.},
title={Efficient Parallel and Out of Core Algorithms for Constructing Large Bi-directed de Bruijn Graphs},
key={arXiv:1003.1940 [cs.DS]},
note={\url{http://arxiv.org/abs/1003.1940}},
year={2010},
month={March}
}
@unpublished{np-hard-blm,
author={Kundeti,V. and Rajasekaran,S. and Dihh,H.},
title={On the Border Length Minimization Problem (BLMP) on a Square Array},
key={arXiv:1003.2839 [cs.DS]},
note={\url{http://arxiv.org/abs/1003.2839}},
year={2010},
month={January}
}

@inproceedings{bibe_hardness,
author={Kundeti,V. and Rajasekaran,S.},
editor={ },
year={2009},
title={On the hardness of the border length minimization problem},
booktitle={9th IEEE International Conference on Bioinformatics and Bioengineering (BIBE)},
pages={248-253}
}

@incollection{isbra_self_assembly,
author={Kundeti,V. and Rajasekaran,S.},
year={2009},
title={Efficient algorithms for self assembling triangular and other nano structures},
booktitle = {Springer LNCS},
volume={5542},
pages={148-158}
}

@article{graph_isomorphism,
author={Rajasekaran,S. and Kundeti,V.},
year={2009},
title={Spectrum based techniques for graph isomorphism},
journal={International Journal of Foundations of Computer Science},
volume={20},
number={3},
pages={479-499}
}

@article{mnm2_system,
author={Rajasekaran,S. and Balla,S. and Gradie,P. and Gryk,M. R. and Kadaveru,K. and Kundeti,V. and Maciejewski,M. W. and Mi,T. and Rubino,N. and Vyas,J. and Schiller,M. R.},
year={2009},
title={Minimotif miner 2nd release: A database and web system for motif search},
journal={Nucleic acids research},
volume={37},
number={SUPPL. 1},
pages={D185-D190}
}

@inproceedings{protein_structure,
author={Kundeti,V. and Rajasekaran,S.},
year={2008},
title={A local structural alignment algorithm with variable length alignment fragment Pairs},
booktitle={8th IEEE International Conference on Bioinformatics and Bioengineering (BIBE) },
pages={1-7}
}

@book{hipc08,
author={Kundeti,V. and Rajasekaran,S.},
year={2008},
title={Efficient PDM sorting algorithms},
volume={5374 LNCS},
pages={97-107}
}

@inproceedings{asap08,
author={Kundeti,V. and Fei,Y. and Rajasekaran,S.},
year={2008},
title={An efficient digital circuit for implementing sequence alignment algorithm in an extended processor},
pages={156-161},
booktitle={19th IEEE International Conference on Application-specific Systems, Architectures and Processors (ASAP)}
}


@incollection{four_russian,
author={Kundeti,V. and Rajasekaran,S.},
year={2008},
title={Extending the four Russian algorithm to compute the edit script in linear space},
booktitle={Springer LNCS},
volume={5101},
number={PART 1},
pages={893-902}
}

@article{vlsi_layout,
author={Kundeti,V. K. and Gupta,P.},
year={2006},
title={Optimal algorithms for some polygon enclosure problems for VLSI Layout Analysis},
journal={Journal of Mathematical Modelling and Algorithms},
volume={5},
number={3},
pages={259-271}
}


@article{hgp_project,
	author={Lander,E. S. and Linton,L. M. and Birren,B. and Nusbaum,C. and Zody,M. C. et al}, 
	year={2001},
	title={Initial sequencing and analysis of the human genome},
	journal={Nature},
	volume={409},
	number={6822},
	pages={860-921}
}







@article{hgp_project_long,
	author={Lander,E. S. and Linton,L. M. and Birren,B. and Nusbaum,C. and Zody,M. C. and Baldwin,J. and Devon,K. and Dewar,K. and Doyle,M. and Fitzhugh,W. and Funke,R. and Gage,D. and Harris,K. and Heaford,A. and Howland,J. and Kann,L. and Lehoczky,J. and Levine,R. and McEwan,P. and McKernan,K. and Meldrim,J. and Mesirov,J. P. and Miranda,C. and Morris,W. and Naylor,J. and Raymond,C. and Rosetti,M. and Santos,R. and Sheridan,A. and Sougnez,C. and Stange-Thomann,N. and Stojanovic,N. and Subramanian,A. and Wyman,D. and Rogers,J. and Sulston,J. and Ainscough,R. and Beck,S. and Bentley,D. and Burton,J. and Clee,C. and Carter,N. and Coulson,A. and Deadman,R. and Deloukas,P. and Dunham,A. and Dunham,I. and Durbin,R. and French,L. and Grafham,D. and Gregory,S. and Hubbard,T. and Humphray,S. and Hunt,A. and Jones,M. and Lloyd,C. and McMurray,A. and Matthews,L. and Mercer,S. and Milne,S. and Mullikin,J. C. and Mungall,A. and Plumb,R. and Ross,M. and Shownkeen,R. and Sims,S. and Waterston,R. H. and Wilson,R. K. and Hillier,L. W. and McPherson,J. D. and Marra,M. A. and Mardis,E. R. and Fulton,L. A. and Chinwalla,A. T. and Pepin,K. H. and Gish,W. R. and Chissoe,S. L. and Wendl,M. C. and Delehaunty,K. D. and Miner,T. L. and Delehaunty,A. and Kramer,J. B. and Cook,L. L. and Fulton,R. S. and Johnson,D. L. and Minx,P. J. and Clifton,S. W. and Hawkins,T. and Branscomb,E. and Predki,P. and Richardson,P. and Wenning,S. and Slezak,T. and Doggett,N. and Cheng,J. -. and Olsen,A. and Lucas,S. and Elkin,C. and Uberbacher,E. and Frazier,M. and Gibbs,R. A. and Muzny,D. M. and Scherer,S. E. and Bouck,J. B. and Sodergren,E. J. and Worley,K. C. and Rives,C. M. and Gorrell,J. H. and Metzker,M. L. and Naylor,S. L. and Kucherlapati,R. S. and Nelson,D. L. and Weinstock,G. M. and Sakaki,Y. and Fujiyama,A. and Hattori,M. and Yada,T. and Toyoda,A. and Itoh,T. and Kawagoe,C. and Watanabe,H. and Totoki,Y. and Taylor,T. and Weissenbach,J. and Heilig,R. and Saurin,W. and Artiguenave,F. and Brottier,P. and Bruls,T. and Pelletier,E. and Robert,C. and Wincker,P. and Rosenthal,A. and Platzer,M. and Nyakatura,G. and Taudien,S. and Rump,A. and Smith,D. R. and Doucette-Stamm,L. and Rubenfield,M. and Weinstock,K. and Hong,M. L. and Dubois,J. and Yang,H. and Yu,J. and Wang,J. and Huang,G. and Gu,J. and Hood,L. and Rowen,L. and Madan,A. and Qin,S. and Davis,R. W. and Federspiel,N. A. and Abola,A. P. and Proctor,M. J. and Roe,B. A. and Chen,F. and Pan,H. and Ramser,J. and Lehrach,H. and Reinhardt,R. and McCombie,W. R. and De La Bastide,M. and Dedhia,N. and Blöcker,H. and Hornischer,K. and Nordsiek,G. and Agarwala,R. and Aravind,L. and Bailey,J. A. and Bateman,A. and Batzoglou,S. and Birney,E. and Bork,P. and Brown,D. G. and Burge,C. B. and Cerutti,L. and Chen,H. -. and Church,D. and Clamp,M. and Copley,R. R. and Doerks,T. and Eddy,S. R. and Eichler,E. E. and Furey,T. S. and Galagan,J. and Gilbert,J. G. R. and Harmon,C. and Hayashizaki,Y. and Haussler,D. and Hermjakob,H. and Hokamp,K. and Jang,W. and Johnson,L. S. and Jones,T. A. and Kasif,S. and Kaspryzk,A. and Kennedy,S. and Kent,W. J. and Kitts,P. and Koonin,E. V. and Korf,I. and Kulp,D. and Lancet,D. and Lowe,T. M. and McLysaght,A. and Mikkelsen,T. and Moran,J. V. and Mulder,N. and Pollara,V. J. and Ponting,C. P. and Schuler,G. and Schultz,J. and Slater,G. and Smit,A. F. A. and Stupka,E. and Szustakowki,J. and Thierry-Mieg,D. and Thierry-Mieg,J. and Wagner,L. and Wallis,J. and Wheeler,R. and Williams,A. and Wolf,Y. I. and Wolfe,K. H. and Yang,S. -. and Yeh,R. -. and Collins,F. and Guyer,M. S. and Peterson,J. and Felsenfeld,A. and Wetterstrand,K. A. and Myers,R. M. and Schmutz,J. and Dickson,M. and Grimwood,J. and Cox,D. R. and Olson,M. V. and Kaul,R. and Raymond,C. and Shimizu,N. and Kawasaki,K. and Minoshima,S. and Evans,G. A. and Athanasiou,M. and Schultz,R. and Patrinos,A. and Morgan,M. J.},
	year={2001},
	title={Initial sequencing and analysis of the human genome},
	journal={Nature},
	volume={409},
	number={6822},
	pages={860-921}
}

@article{celera_project,
	author={Craig Venter,J. and Adams,M. D. and Myers,E. W. and Li,P. W. and Mural,R. J. et.al.}, 
	year={2001},
	title={The sequence of the human genome},
	journal={Science},
	volume={291},
	number={5507},
	pages={1304-1351}
}








@article{celera_project1,
	author={Craig Venter,J. and Adams,M. D. and Myers,E. W. and Li,P. W. and Mural,R. J. and Sutton,G. G. and Smith,H. O. and Yandell,M. and Evans,C. A. and Holt,R. A. and Gocayne,J. D. and Amanatides,P. and Ballew,R. M. and Huson,D. H. and Wortman,J. R. and Zhang,Q. and Kodira,C. D. and Zheng,X. H. and Chen,L. and Skupski,M. and Subramanian,G. and Thomas,P. D. and Zhang,J. and Gabor Miklos,G. L. and Nelson,C. and Broder,S. and Clark,A. G. and Nadeau,J. and McKusick,V. A. and Zinder,N. and Levine,A. J. and Roberts,R. J. and Simon,M. and Slayman,C. and Hunkapiller,M. and Bolanos,R. and Delcher,A. and Dew,I. and Fasulo,D. and Flanigan,M. and Florea,L. and Halpern,A. and Hannenhalli,S. and Kravitz,S. and Levy,S. and Mobarry,C. and Reinert,K. and Remington,K. and Abu-Threideh,J. and Beasley,E. and Biddick,K. and Bonazzi,V. and Brandon,R. and Cargill,M. and Chandramouliswaran,I. and Charlab,R. and Chaturvedi,K. and Deng,Z. and Di Francesco,V. and Dunn,P. and Eilbeck,K. and Evangelista,C. and Gabrielian,A. E. and Gan,W. and Ge,W. and Gong,F. and Gu,Z. and Guan,P. and Heiman,T. J. and Higgins,M. E. and Ji,R. -. and Ke,Z. and Ketchum,K. A. and Lai,Z. and Lei,Y. and Li,Z. and Li,J. and Liang,Y. and Lin,X. and Lu,F. and Merkulov,G. V. and Milshina,N. and Moore,H. M. and Naik,A. K. and Narayan,V. A. and Neelam,B. and Nusskern,D. and Rusch,D. B. and Salzberg,S. and Shao,W. and Shue,B. and Sun,J. and Zhen Yuan Wang and Wang,A. and Wang,X. and Wang,J. and Wei,M. -. and Wides,R. and Xiao,C.},
	year={2001},
	title={The sequence of the human genome},
	journal={Science},
	volume={291},
	number={5507},
	pages={1304-1351}
}

@unpublished{bi-appx-2010,
AUTHOR={V. Kundeti and S. Rajasekaran},
TITLE={Approximation Algorithms for Shortest Double Stranded DNA String Problem},
NOTE={(under review)},
YEAR={2010}
}

@article{directed_cpp,
author = {Papadimitriou, Christos H.},
title = {On the complexity of edge traversing},
journal = {J. ACM},
volume = {23},
issue = {3},
month = {July},
year = {1976},
issn = {0004-5411},
pages = {544--554},
numpages = {11},
url = {http://doi.acm.org/10.1145/321958.321974},
doi = {http://doi.acm.org/10.1145/321958.321974},
acmid = {321974},
publisher = {ACM},
address = {New York, NY, USA},
}

@ARTICLE{drake03,
author = {Doratha E. Drake and Stefan Hougardy},
title = {A Simple Approximation Algorithm for the Weighted Matching Problem},
journal = {Information Processing Letters},
year = {2003},
volume = {85},
pages = {211--213}
}

